CN-DHF: Compact Neural Double Height-Field Representations of 3D Shapes

We introduce CN-DHF (Compact Neural Double-Height-Field), a novel hybrid neural implicit 3D shape representation that is dramatically more compact than the current state of the art. Our representation leverages Double-Height-Field (DHF) geometries, defined as closed shapes bounded by a pair of oppositely oriented height-fields that share a common axis, and leverages the following key observations: DHFs can be compactly encoded as 2D neural implicits that capture the maximal and minimal heights along the DHF axis; and typical closed 3D shapes are well represented as intersections of a very small number (three or fewer) of DHFs. We represent input geometries as CNDHFs by first computing the set of DHFs whose intersection well approximates each input shape, and then encoding these DHFs via neural fields. Our approach delivers high-quality reconstructions, and reduces the reconstruction error by a factor of 2:5 on average compared to the state-of-the-art, given the same parameter count or storage capacity. Compared to the best-performing alternative, our method produced higher accuracy models on 94% of the 400 input shape and parameter count combinations tested.

==> 5-implementation.tex <==
\section{Implementation}
\label{sec:implementation}

Implementation


Our Method
==========

Input: mesh M and parameter count P

Steps:

1.  Compute the minimal and sufficient set of DHF directions, let N be the number of output directions.

2. (DEBUG) Use the input mesh + the N directions in Eric code to  generate 2 * N "ground truth" HF meshes (the ones with a flat extent outside).

3. Train N models each using P/N parameters using the provided information,  save the models at 10K, 100K, and 1M iterations (record training times).

4. Export the 2 * HF meshes using the trained models.

5. Directly render the shapes defined by the intersection of our N models.

6. Directly measure chamfer + IoU between our output (intersection of N models) and our input mesh M

7. Either matchingclube our intersection of N models or tetWild the output of number 4 (after removing redundant triangles).  Measure Hausdorf distance vs input M.


Other Methods:
=============

0. Compress the outputs of stage 4 of our method using JPG (see how to define parameters/mesh size).

1. Setup/Run NGLOD with P parameters

2. Setup/Run SIREN with P parameters

3. Setup/Run InstantNGP with P parameters

4.  For each of the above measure chamfer vs ground truth using the same method as for us.

5.  For each of the above measure IoU vs ground truth using the same method as for us.

6.  For each of the above export marching cubes mesh and measure Hausdorf distance  vs ground truth using the same method as for us.

7. 4.  For each of the above visualize the output (implicit and mesh).


Data
====

1. Use our 100 inputs so far.

2. Add ALL inputs from NGLOD paper.

3. Look at SIREN and InstantNGP papers and add more inputs from there.

4. Add inputs from ShapeNet - especially useful for human made stuff which is a single dhf.  We need the clean ShapeNet models (Wenping Wang? Or?)

5.  At the very least we can for all these inputs (and some subset of classes of ShapeNet?) measure how many dhf directions they require.  This is an important statistics, even if we do not train models for all these inputs.

==> tables/l1vl2.tex <==
\begin{table}
    \caption{\TODO{unsure if below or above!}\TODO{loss function design table -- low priority}\TODO{Note I am using graphics, but this really should be a table}}
    \label{tab:l1vl2}
    \includegraphics[width=\linewidth]{figures/example-image-a-wide.png}
\end{table}
